Minimax-Optimal Predictive Flow Matching under Distribution Drift

Flow matching learns a generative velocity field by regression, but under distribution drift a field must be deployed before the current data arrive. We study this predictive problem for a fixed, possibly nonconvex, neural class, with dynamic regret against the best represented field of each round. We propose DyProd-FM, which refits flow matching on dyadic historical prefixes and selects among the fits with a sleeping Prod master. Without knowing any drift budget, it attains regret $\widetilde{O}(\min\{N_\omega+1,1+\sqrt{T\Omega}\})$ in the relative velocity risk variation $\Omega$ and $\widetilde{O}(\min\{N_\mu+1,1+T^{1/3}V_\mu^{2/3}\})$ in the target-law variation $V_\mu=\sum_t W_2(\mu_{t+1},\mu_t)$, up to approximation and fitting costs. Matching lower bounds for fixed classes show that both rates are optimal in $T$ and in the budgets up to logarithmic factors. Prior optimal dynamic-regret guarantees rely on a convex decision set with strongly convex or exp-concave losses, whereas our class may be nonconvex and no curvature in its parameters is assumed. The target-law rate rests on a second-order link between the two variations, which the base noise of flow matching provides.

==> appendices/setup.tex <==
\appendix
\renewcommand{\theequation}{\arabic{equation}}
\makeatletter
\setcounter{theorem}{0}\renewcommand{\thetheorem}{\thesection.\arabic{theorem}}\@addtoreset{theorem}{section}
\setcounter{lemma}{0}\renewcommand{\thelemma}{\thesection.\arabic{lemma}}\@addtoreset{lemma}{section}
\setcounter{proposition}{0}\renewcommand{\theproposition}{\thesection.\arabic{proposition}}\@addtoreset{proposition}{section}
\setcounter{corollary}{0}\renewcommand{\thecorollary}{\thesection.\arabic{corollary}}\@addtoreset{corollary}{section}
\setcounter{remark}{0}\renewcommand{\theremark}{\thesection.\arabic{remark}}\@addtoreset{remark}{section}
\setcounter{assumption}{0}\renewcommand{\theassumption}{\thesection.\arabic{assumption}}\@addtoreset{assumption}{section}
\makeatother
% ===== Original supplement.tex =====
\begin{center}
{\Large\bfseries Minimax-Optimal Predictive Flow Matching under Distribution Drift}\\[5pt]
{\large Supplementary Material}
\end{center}

